CoQuest: Exploring Research Question Co-Creation with an LLM-based Agent

Developing novel research questions (RQs) often requires extensive literature reviews, especially in interdisciplinary fields. To support RQ development through human-AI co-creation, we leveraged Large Language Models (LLMs) to build an LLM-based agent system named CoQuest. We conducted an experiment with 20 HCI researchers to examine the impact of two interaction designs: breadth-first and depth-first RQ generation. The findings revealed that participants perceived the breadth-first approach as more creative and trustworthy upon task completion. Conversely, during the task, participants considered the depth-first generated RQs as more creative. Additionally, we discovered that AI processing delays allowed users to reflect on multiple RQs simultaneously, leading to a higher quantity of generated RQs and an enhanced sense of control. Our work makes both theoretical and practical contributions by proposing and evaluating a mental model for human-AI co-creation of RQs. We also address potential ethical issues, such as biases and over-reliance on AI, advocating for using the system to improve human research creativity rather than automating scientific inquiry.

==> backup/3-formative.tex <==
\section{Formative Study}
We first conducted a formative study to understand the cognitive process of researchers creating research questions. 
To understand how researchers create RQs, we first conducted semi-structured interviews with 4 researchers about their research process; 
We then organized a focus group with the interviewed participants to identify their needs for an RQ generation system. 

\subsection{Formative Interview}
We invited four researchers to participate in our semi-structured interviews, in order to understand their process of conducting research. All 4 participants are doctoral researchers. 
We ask the interviewees to describe their most recent experience working on a research project from scratch. 

\textbf{Iterative ideation through literature survey} 
Most participants mentioned starting from a rough idea (e.g., domains, keywords, application scenarios) before searching for related literature. 
Participants also emphasized that formulating research ideas is often an iterative process. Typically, participants used one or multiple hypothetical research questions/ideas to facilitate the search for related literature and identify research gaps. Then, the research questions/ideas can be revised based on the retrieved literature and research gaps. The two-step process is performed repetitively, continuously refining the research questions/ideas. 


\textbf{Hierarchical question formulation}
Participants also identified their process of research question creation as hierarchical. 
One participant explicitly mentioned that creating research questions naturally resembles the form of a ``mind map'', where the development of ideas gradually ``narrows down'' but could have different branches. 
As described by the participant, the initial set of RQs can often be broader and more general and can subsequently derive sub-RQs under the topics of their predecessors, which helps facilitate the trade-off between specific and general ideas as a common decision-making step during the research ideation process.
This process often results in the evolution of RQs that, when visualized, can be drawn as a tree of RQs. This later informed the design of our system to take the form of an interactive ``mind map'' that preserves the provenance of RQ development. 

% \textbf{The trade-off of specificity}
% Participants mentioned the trade-off between specific and general ideas as a common decision-making step during the research ideation process. 



Additionally, by understanding participants' workflow of creating new research ideas and identifying challenges they encounter, we also identified three major challenges in their research idea creation process:
\yiren{Only include what the system can address here}
\begin{circledenum}
    \item Novice researchers have challenges in identifying good related work.
    \item Researchers find it hard to identify gaps between their ideas and existing work.
    \item Novice researchers have difficulties in evaluating the quality of research ideas.
\end{circledenum}



% \yiren{This yields the mental model}




\textbf{Mental Model of RQ Formulation}
\label{sec:mental_model}
One of the challenges in designing AI-based systems is the violation of users' existing mental models \cite{weisz2023toward}. 
In this study, we designed our system based on the mental model of how researchers create new research ideas by combining existing literature with the findings from our formative interview. 

% \yiren{[EXPLAIN THE PROCESS OF MENTAL MODEL CREATION]}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{img/mentalModel.png}
    \caption{
    Humans' mental model of RQ co-creation with the LLM-based agent.
    \yiren{
    add an AI component in the mental model, in the discussion section, by color coding the different actions; Then claim this is a Human-AI co-creation mental model, and move to the end; 
    Add a verb to each beginning of action, and underscore them; 
    } }
    \label{fig:mental_model}
\end{figure}

The proposed mental model consists of three major components: \textbf{Literature Discovery}, \textbf{Research Question Creation}, and \textbf{Research Question Evaluation}. 
Past research has provided in-depth discussion over how literature discovery plays a major role in the scientific research process \cite{foster2004nonlinear,palmer2009scholarly}. \yiren{TODO}
However, refining research questions has often been interpreted as a sub-step of literature search and understanding. Although research ideation and literature search are mutually dependent, our formative study results indicated a distinction between the behaviors researchers conducted during the two different stages.
By proposing a new mental model, we aim to explicate researchers' behavior of idea creation from literature discovery. 
\yiren{Link major activities with existing literature, and what is newly supported by us}


\subsection{Focus Group}
\yiren{This yields the design requirements}

With the discovered mental model from our formative study, we seek to design an AI-based system that supports users' research question creation process. 
In order to understand how such a system can be designed to assist users' existing workflow, we conducted a focus group study with 4 participants to 1) further understand their interactions when creating new research questions; 2) discover their needs and how an AI-based system can be designed to support the needs. 



% The focus group begins by showing the participants the persona of a novice researcher who has recently come up with a general research idea about a certain topic, and wants to continue on making the research goal more specific and conduct further research steps.



\begin{figure}[th]
    \centering
    \begin{subfigure}{.4\textwidth}
        \centering
        \begin{adjustbox}{valign=c}
            \includegraphics[width=.95\linewidth]{img/focusGroup1.png}
        \end{adjustbox}
    \end{subfigure}%
    \begin{subfigure}{.6\textwidth}
        \centering
        \begin{adjustbox}{valign=c}
            \includegraphics[width=.95\linewidth]{img/focusGroup2.png}
        \end{adjustbox}
    \end{subfigure}
    \caption{
    The co-designed results created by participants during the focus group.
    \yun{this figure is a little bit hard to read. what's the purpose of this figure? I feel the left part of the figure can be written in text, since people won't be able to read the texts in the post-its. is the right figure for } 
    \yiren{Here I mainly want to give a sneak peek of the two-step focus group: 1) brainstorming design needs with 3 questions are cues; 2) co-designing a workflow ; 
    But I don't want to give too much detail here either, since it is not our major contribution.}
    }
    \label{fig:focus_group}
\end{figure}


The focus group was conducted in a two-step process. First, provided with three questions created by researchers as cues, participants were asked to brainstorm ideas and design expectations given the context of an AI-based system that supports research question development. The three question cues were designed as follows: 1) What questions will you ask the AI system? 2) What information do you want to provide for the model to generate RQ for you? 3) How do you produce RQ currently? And do you think the AI model can help you produce RQs?
After discussion and summarizing themes, participants were asked to proceed to the second stage, where they co-design a hypothetical workflow by contextualizing themselves using an AI-based RQ generation system.
During the focus group, we found that participants highlighted several expectations for designing a human-AI RQ co-creation system: 
\begin{itemize}
    \item \textbf{Control:}  
\end{itemize}
\yiren{TODO}
\yiren{Add that users mention the importance of generating different variation of outcomes}



Based on our findings from the focus group, we propose the following design requirements for the system:
\begin{itemize}
    \item[] \textbf{[D1]} Assist users' brainstorming process by automatically generating RQ candidates by taking human feedback
    \item[] \textbf{[D2]} Explain AI rationale
    \item[] \textbf{[D3]} Help users discover relevant literature and identify research gaps
\end{itemize}



